TransientTables: Evaluating LLMs' Reasoning on Temporally Evolving Semi-structured Tables

Humans continuously make new discoveries, and understanding temporal sequence of events leading to these breakthroughs is essential for advancing science and society. This ability to reason over time allows us to identify future steps and understand the effects of financial and political decisions on our lives. However, large language models (LLMs) are typically trained on static datasets, limiting their ability to perform effective temporal reasoning. To assess the temporal reasoning capabilities of LLMs, we present the TRANSIENTTABLES dataset, which comprises 3,971 questions derived from over 14,000 tables, spanning 1,238 entities across multiple time periods. We introduce a template-based question-generation pipeline that harnesses LLMs to refine both templates and questions. Additionally, we establish baseline results using state-of-the-art LLMs to create a benchmark. We also introduce novel modeling strategies centered around task decomposition, enhancing LLM performance.

==> Motivation.tex <==
\paragraph{Why the study of semi-structed data?} Semi-structured tables are everywhere in this modern world from web pages to nutrition tables on food products. Semi-structured data, in contrast to structured data, such as databases is not characterized by pre-defined schemas. Unlike fully structured data (such as SQL databases or knowledge graphs) or unstructured text, entity-centric tables like Wikipedia Infoboxes are unique in that they combine elements of structured and unstructured data. While they offer a degree of structure, their information is often stored in implicit forms, making them more flexible than traditional databases or knowledge graphs. Tables are powerful tools for organizing and visualizing temporal information, particularly when studying an entity's evolution over time. By presenting information in a systematic, organized manner, tables not only serve as comprehensive historical records but also facilitate temporal reasoning and analysis, making it easier to understand how different attributes of an entity have developed throughout its history.

\paragraph{The ever changing nature of information }presents a unique challenge in our digital age, where data is constantly evolving, being updated, and requiring revision. In this dynamic landscape, semi-structured data like Wikipedia Infoboxes have emerged as remarkably adaptable vessels for capturing and reflecting these ongoing changes. Unlike rigid databases that struggle with frequent updates or unstructured text that can become unwieldy and difficult to parse, these tables strike an elegant balance that is flexible enough to accommodate new information while maintaining sufficient structure to remain organized. As entities evolve, whether public figures taking on new roles, companies pivoting their strategies, or scientific concepts being refined, the Infoboxes evolve with them, serving as living documents that reflect the fluid nature of information. Their semi-structured nature allows for quick updates while preserving historical context, making them invaluable tools to document and understand the constant flux of information in the modern world.
